Fashion Image-to-Image Translation for Complementary Item Retrieval

The increasing demand for online fashion retail has boosted research in fashion compatibility modeling and item retrieval, focusing on matching user queries (textual descriptions or reference images) with compatible fashion items. A key challenge is top-bottom retrieval, where precise compatibility modeling is essential. Traditional methods, often based on Bayesian Personalized Ranking (BPR), have shown limited performance. Recent efforts have explored using generative models in compatibility modeling and item retrieval, where generated images serve as additional inputs. However, these approaches often overlook the quality of generated images, which could be crucial for model performance. Additionally, generative models typically require large datasets, posing challenges when such data is scarce. To address these issues, we introduce the Generative Compatibility Model (GeCo), a two-stage approach that improves fashion image retrieval through paired image-to-image translation. First, the Complementary Item Generation Model (CIGM), built on Conditional Generative Adversarial Networks (GANs), generates target item images (e.g., bottoms) from seed items (e.g., tops), offering conditioning signals for retrieval. These generated samples are then integrated into GeCo, enhancing compatibility modeling and retrieval accuracy. Evaluations on three datasets show that GeCo outperforms state-of-the-art baselines. Key contributions include: (i) the GeCo model utilizing paired image-to-image translation within the Composed Image Retrieval framework, (ii) comprehensive evaluations on benchmark datasets, and (iii) the release of a new Fashion Taobao dataset designed for top-bottom retrieval, promoting further research.

==> tables/box_plots.tex <==


% Define colors
\definecolor{myblue}{RGB}{31, 119, 180}
\definecolor{myred}{RGB}{214, 39, 40}

\begin{tikzpicture}
    \begin{axis}[
        width=12cm,  % Adjust width as needed
        height=8cm,  % Adjust height as needed
        boxplot/draw direction=y,
        boxplot/whisker range=4.5,  % Adjust whisker range as needed
        boxplot/every whisker/.style={very thick},
        boxplot/every box/.style={fill=myblue!50},
        boxplot/every median/.style={very thick, draw=myblue},
        xlabel={Hyperparameter},
        ylabel={Metric},
        xtick={1, 2, 3},  % Adjust x-axis ticks according to your data
        xticklabels={Alpha, Beta, Temperature},  % Labels for x-axis ticks
        x tick label style={text width=2cm, align=center},
        yticklabel style={font=\small},
        enlarge x limits=0.5,  % Adjust spacing at the ends of x-axis
        font=\footnotesize,
        title style={font=\bfseries, yshift=-1ex},
        title={Boxplot of Metric vs. Hyperparameter},
        legend style={at={(0.5,-0.15)}, anchor=north, legend columns=-1},
        legend image code/.code={%
            \draw[#1, line width=0.6pt] (-0.3cm,0cm) rectangle ++(0.6cm,0.15cm);
        },
    ]
    
    % Load data from CSV file
    \pgfplotstableread[col sep=comma]{hp_pog.csv}\datatable

    % Boxplot for AUC_1vs1
    \addplot+[boxplot] table[y=AUC_1vs1, col sep=comma] {\datatable};
    \addlegendentry{AUC\_1vs1}
    
    % Boxplot for MRR_1vsall
    \addplot+[boxplot] table[y=MRR_1vsall, col sep=comma] {\datatable};
    \addlegendentry{MRR\_1vsall (10\textsuperscript{-2})}
    
    \end{axis}
\end{tikzpicture}

